Adversarial Attacks on GMM i-vector based Speaker Verification Systems

This work investigates the vulnerability of Gaussian Mixture Model (GMM) i-vector based speaker verification systems to adversarial attacks, and the transferability of adversarial samples crafted from GMM i-vector based systems to x-vector based systems. In detail, we formulate the GMM i-vector system as a scoring function of enrollment and testing utterance pairs. Then we leverage the fast gradient sign method (FGSM) to optimize testing utterances for adversarial samples generation. These adversarial samples are used to attack both GMM i-vector and x-vector systems. We measure the system vulnerability by the degradation of equal error rate and false acceptance rate. Experiment results show that GMM i-vector systems are seriously vulnerable to adversarial attacks, and the crafted adversarial samples prove to be transferable and pose threats to neuralnetwork speaker embedding based systems (e.g. x-vector systems).

==> adversarial attacks on GMM i-vector based speaker verification systems/abstract-keywords.tex <==
\begin{abstract}
This work investigates the vulnerability of Gaussian Mixture Model (GMM) i-vector based speaker verification systems to adversarial attacks, and the transferability of adversarial samples crafted from GMM i-vector based systems to x-vector based systems. 
% In detail, we formulate the GMM i-vector based system as a scoring function, and leverage the fast gradient sign method (FGSM) to generate adversarial samples through this function. 
In detail, we formulate the GMM i-vector system as a scoring function of enrollment and testing utterance pairs. Then we leverage the fast gradient sign method (FGSM) to optimize testing utterances for adversarial samples generation.
These adversarial samples are used to attack both GMM i-vector and x-vector systems. We measure the system vulnerability by the degradation of equal error rate and false acceptance rate. Experiment results show that GMM i-vector systems are seriously vulnerable to adversarial attacks, and the crafted adversarial samples prove to be transferable and pose threats to neural network speaker embedding based systems (e.g. x-vector systems).
\end{abstract}
%
\begin{keywords}
Adversarial attack, speaker verification, GMM i-vector, x-vector
\end{keywords}


==> adversarial attacks on GMM i-vector based speaker verification systems/acknowledgement.tex <==
\section{acknowledgement}
This work is partially supported by HKSAR Government's Research Grants Council General Research Fund (Project No. 14208718).


==> adversarial attacks on GMM i-vector based speaker verification systems/adv-examples-gen.tex <==
\section{adversarial samples generation}
\label{sec:adv-examples-gen}

In this work, we investigate the vulnerability of ASV systems to adversarial attacks, including the white box attack and black box attacks in terms of cross-feature, cross-model architecture and cross-feature-model settings. Three ASV models are well-trained in our experiments: Mel-frequency cepstral coefficient (MFCC) based GMM i-vector system (MFCC-ivec), log power magnitude spectrum (LPMS) based GMM i-vector system (LPMS-ivec) and MFCC based x-vector system (MFCC-xvec). The white box attack and black box mutual attack settings are illustrated in Fig.~\ref{fig:adv-attack-config}. Two white box attacks are performed on MFCC-ivec and LPMS-ivec systems, respectively. The three black box attack settings are designed as follows: LPMS-ivec attacks MFCC-ivec (cross-feature), MFCC-ivec attacks MFCC-xvec (cross-model architecture) and LPMS-ivec attacks MFCC-xvec (cross-feature-model). The last two settings are to investigate the transferability of adversarial samples crafted from GMM i-vector systems to x-vector systems.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{adv-attack-config-new.png}
    \caption{The adversarial attack configuration. Each arrow represents an attack setting, where it points from the source model to the target model.}
    \label{fig:adv-attack-config}
\end{figure}

To perform the attacks above, adversarial samples need to be crafted from the source models, i.e. LPMS-ivec and MFCC-ivec in our case. In this work, we generate adversarial samples at the acoustic feature level, i.e. either MFCC or LPMS. In the black box attacks of cross-feature and cross-feature-model settings, the generated adversarial features (LPMS) are first inverted to audios, then the acoustic features adopted in the target models are extracted from the audios to perform attacks. In other cases, the adversarial features could be directly used for attacks.
% To perform an adversarial attack, we regard the target system parameters as fixed and optimize over the input space to search an adversarial solution. Specifically, we search for a small perturbation $\delta_x$ to be added on original signal $x$, as Equation \ref{eq:x-star}. This perturbation is as small as human ears can not distinguish the adversarial audios from original ones.

% Formally, we denote the system parameters as $\theta$, the system function as f, and input and output as x and y respectively. L is the loss function between system output and ground truth y. Then we maximize L with the constrain that the p norm of $\delta_x$ is within a perturbation degree $\epsilon$. The formal equation lies in Equation \ref{eq:formal-adv}.

\subsection{Fast gradient sign method}
In a general case, we denote a system function as $f$ with parameters $\theta$. Given the original input $\boldsymbol{x}$, we search for an adversarial perturbation $\boldsymbol{\delta_x}$ to be added to $\boldsymbol{x}$ to generate the adversarial sample $\boldsymbol{x^\star} = \boldsymbol{x} + \boldsymbol{\delta_x}$. This adversarial perturbation $\boldsymbol{\delta_x}$ is optimized by maximizing the deviation between the system's prediction given adversarial input $\boldsymbol{x^\star}$ and the ground truth $y$, as shown in Eq.~\ref{eq:formal-adv},
\begin{equation}
    \boldsymbol{\delta_x} = \arg\max_{\Vert \boldsymbol{\delta_x} \Vert_p \leq \epsilon} L(f_{\theta}(\boldsymbol{x}+\boldsymbol{\delta_x}), y)
    \label{eq:formal-adv}
\end{equation}
The deviation is measured by a loss function $L$ between the system prediction and the ground truth, which is usually adopted as either cross entropy for classification tasks or mean square error for regression tasks. The $p$-norm constraint on $\boldsymbol{\delta_x}$ guarantees that human cannot distinguish the adversarial sample $\boldsymbol{x^\star}$ from the original $\boldsymbol{x}$, and the upper bound $\epsilon$ represents the perturbation degree. Note that the system parameters $\theta$ are always fixed during the optimization procedure, which means adversarial attackers only revise the input to attack systems instead of the system parameters.

% Many algorithms were previously proposed to solve the optimization problem in Eq.~\ref{eq:formal-adv}, such as fast gradient sign method (FGSM) \cite{goodfellow2014explaining}, basic iterative method (BIM) \cite{kurakin2016adversarial} and DeepFool \cite{moosavi2016deepfool}. In this work, we only adopt a simple method, i.e. FGSM, to verify the ASV system's vulnerability to adversarial attacks.

% In a general case, we denote a system function as $f$ with parameters $\theta$. Given the input $\boldsymbol{x}$, we search for an adversarial perturbation $\boldsymbol{\delta_x}$ to be added to $\boldsymbol{x}$ for maximizing the loss function $L$ between the system's prediction and ground truth $y$, as shown in Eq.~\ref{eq:formal-adv},
% \begin{equation}
%     \boldsymbol{\delta_x} = \arg\max_{\Vert \boldsymbol{\delta_x} \Vert_p \leq \epsilon} L(f_{\theta}(\boldsymbol{x}+\boldsymbol{\delta_x}), y)
%     \label{eq:formal-adv}
% \end{equation}
% Note that the system parameters $\theta$ are fixed and we revise the input $\boldsymbol{x}$ to maximize the the deviation between the system prediction and the ground truth, to make the system give a wrong prediction. The constraint that the $p$-norm of $\boldsymbol{\delta_x}$ is within a perturbation degree $\epsilon$ guarantees human can not distinguish the adversarial sample $\boldsymbol{x^\star} = \boldsymbol{x} + \boldsymbol{\delta_x}$ from original $\boldsymbol{x}$.


% \begin{equation}
%     x^\star = x + \delta_x
%     \label{eq:x-star}
% \end{equation}

% \subsection{Fast gradient sign method}
% In this work, we specialize p as $\infty$, and use fast sign gradient method (FSGM) to search a suitable solution. FSGM takes a one single step towards the gradient direction, and the step length is perturbation degree $\epsilon$, as shown in Equation \ref{eq:fsgm-adv}.

In this work, we adopt fast gradient sign method (FGSM) \cite{goodfellow2014explaining} to solve the optimization problem in Eq.~\ref{eq:formal-adv}. It perturbs the original input $\boldsymbol{x}$ towards the gradient of the loss function $L$ w.r.t. $\boldsymbol{x}$ to generate adversarial samples. Specifically, it specializes the norm $p$ in Eq.~\ref{eq:formal-adv} as $\infty$, and gives the solution as Eq.~\ref{eq:fsgm-adv},
\begin{equation}
    \boldsymbol{\delta_x} = \epsilon \times sign(\nabla_{\boldsymbol{x}} L(f_{\theta}(\boldsymbol{x}), y))
    \label{eq:fsgm-adv}
\end{equation}
where the function $sign(\cdot)$ takes the sign of the gradient, and $\epsilon$ represents the perturbation degree.

% In this work, fast gradient sign method (FGSM) is adopted to solve Eq.~\ref{eq:formal-adv}, in which the norm $p$ is specialized as $\infty$. The solution is given in Eq.~\ref{eq:fsgm-adv},
% \begin{equation}
%     \boldsymbol{\delta_x} = \epsilon \times sign(\nabla_{\boldsymbol{x}} L(f_{\theta}(\boldsymbol{x}), y))
%     \label{eq:fsgm-adv}
% \end{equation}
% where function $sign(\cdot)$ takes the sign of the gradient. FGSM perturbs $x$ with a small perturbation $\epsilon$ multiplied by the sign of the gradient to generate adversarial samples ($\boldsymbol{x^{\star}}$).

\subsection{Problem formulation}
% In this work, we denote our scoring system as $S$ with parameters $\theta$. During test, each trial consists of one enroll utterance and one test utterance. As mentioned in Section \ref{sec:asv-systems}, the system returns a similarity score between these two utterances. And the system performance, i.e. equal error rate (EER), is estimated over these trial scores. To mimic a realistic model attack, we keep both system parameters and enroll utterance $y_{enroll}$ as fixed, and only revise the test utterance. For target trials, i.e. the enroll and test utterances belong to a same person, we minimize the similarity score whereas for non-target trials, we maximize it. The formulation is shown in Equation \ref{eq:our-case-1} and \ref{eq:our-case-2}.

Adversarial samples are generated from GMM i-vector systems (LPMS-ivec and MFCC-ivec systems). To formulate it into an optimization problem, we denote the GMM i-vector system by two functions: i-vector extractor $f$ with parameters $\theta_1$ and PLDA scoring function $S$ with parameters $\theta_2$. Normalization steps, such as i-vector normalization, are implicitly included within the functions.

The acoustic features of each utterance $i$ are denoted as matrix $\boldsymbol{X_i}$, where each column represents the acoustic feature of each frame and the horizontal axis represents the time sequence. Given the acoustic features of two utterances $\boldsymbol{X_i}$ and $\boldsymbol{X_j}$, the corresponding i-vectors are derived as $\boldsymbol{\omega_i}=f_{\theta_1}(\boldsymbol{X_i})$ and $\boldsymbol{\omega_j}=f_{\theta_1}(\boldsymbol{X_j})$, respectively. Then the final similarity score (PLDA score adopted in our experiments) based on these two i-vectors is derived as $S_{\theta_2}(f_{\theta_1}(\boldsymbol{X_i}), f_{\theta_1}(\boldsymbol{X_j}))$.

In the ASV testing stage, each testing trial consists of one enrollment utterance $\boldsymbol{X_i}$ and one testing utterance $\boldsymbol{X_j}$. According to the speaker identities behind these two utterances, there could be two kinds of trials: target trials and non-target trials. In target trials, the speaker identities behind the enrollment and testing utterances belong to one person. In non-target trials, the identities belong to two different persons. To mimic a realistic model attack, we keep the enrollment features $\boldsymbol{X_i}$ and the system parameters $\{\theta_1, \theta_2\}$ fixed and revise the testing features $\boldsymbol{X_j}$ for adversarial samples generation. For target trials, we search perturbations $\boldsymbol{\delta_X}$ to be added to $\boldsymbol{X_j}$ to minimize the similarity score. For non-target trials, we search perturbations to maximize the score. This could lead the ASV systems to make wrong decisions for both target and non-target trials. The optimization problem formulation is shown in Eq.~\ref{eq:our-case-0}, and the solution given by FGSM is derived as Eq.~\ref{eq:our-case-1} and \ref{eq:our-case-2}.

\begin{align}
    &\boldsymbol{\delta_X} = \arg \max_{\Vert \boldsymbol{\delta_X} \Vert_p \leq \epsilon} k \times S_{\theta_2}(f_{\theta_1}(\boldsymbol{X_i}), f_{\theta_1}(\boldsymbol{X_j}+\boldsymbol{\delta_X})) \label{eq:our-case-0} \\
    &\boldsymbol{\delta_X} = \epsilon \times k \times sign(\nabla_{\boldsymbol{X_j}} S_{\theta_2}(f_{\theta_1}(\boldsymbol{X_i}), f_{\theta_1}(\boldsymbol{X_j}))) \label{eq:our-case-1} \\
    &k = \{ \begin{array}{cc}
     -1, & \text{target trial} \\
     1, & \text{non-target trial}
    \end{array}
    \label{eq:our-case-2}
\end{align}

% In this work, we generate adversarial samples from GMM i-vector systems. We denote the whole system by two parts: i-vector extraction function $f$ with parameter $\theta_1$ and PLDA scoring function $S$ with parameter $\theta_2$. The acoustic feature sequence of each utterance is denoted by $\boldsymbol{X}$. Normalization steps, such as i-vector normalization, are implicitly included within the functions.

% In the testing stage, each trial consists of one enrollment utterance $\boldsymbol{X^{(e)}}$ and one test utterance $\boldsymbol{X}$. To mimic a realistic model attack, we fix $\boldsymbol{X^{(e)}}$ and system parameters $\{\theta_1, \theta_2\}$, and revise $\boldsymbol{X}$ of all trials to perform adversarial attacks. For GMM i-vector framework, there is no explicit ground truth $y$ and loss function $L$ for each output score. We optimize the output score $S$ according to target/non-target trials. For target trials, i.e. the enrollment and test utterances belong to one person, we minimize the similarity score. While for non-target trials, we maximize the score. The problem formulation and its solution are shown in Eq.~\ref{eq:our-case-0}, \ref{eq:our-case-1} and \ref{eq:our-case-2}.

% \begin{align}
%     &\boldsymbol{\delta_X} = \arg \max_{\Vert \boldsymbol{\delta_X} \Vert_p \leq \epsilon} k \times S_{\theta_2}(f_{\theta_1}(\boldsymbol{X}), f_{\theta_1}(\boldsymbol{X^{(e)}})) \label{eq:our-case-0} \\
%     &\boldsymbol{\delta_X} = \epsilon \times k \times sign(\nabla_{\boldsymbol{X}} S_{\theta_2}(f_{\theta_1}(\boldsymbol{X}), f_{\theta_1}(\boldsymbol{X^{(e)}}))) \label{eq:our-case-1} \\
%     &k = \{ \begin{array}{cc}
%      -1, & \text{target trial} \\
%      1, & \text{non-target trial}
%     \end{array}
%     \label{eq:our-case-2}
% \end{align}

% In this work, we measure the vulnerability of the systems to adversarial attacks by the degradation of the systems' equal error rate (EER) and false acceptance rate (FAR). EER is the rate where acceptance and rejection errors are equal. It reflects the balanced system error rate in terms of acceptance and rejection. The FAR threshold is fixed as the EER threshold in the system without attack. FAR reflects the prediction error rate over non-target trials.

% In this work, we train three ASV models: MFCC based GMM i-vector system (MFCC-ivec), LPMS based GMM i-vector system (LPMS-ivec) and MFCC based x-vector system (MFCC-xvec), and perform white and black box attacks. Two white box attacks are performed on MFCC-ivec and LPMS-ivec systems respectively, and three black box attacks in the mutual attack settings: LPMS-ivec attacks MFCC-ivec (cross feature), MFCC-ivec attacks MFCC-xvec (cross model architecture) and LPMS-ivec attacks MFCC-xvec (cross both). The last two settings is to investigate the adversarial samples' transferability to x-vector systems.


==> adversarial attacks on GMM i-vector based speaker verification systems/asv-systems.tex <==
\section{automatic speaker verification systems}
\label{sec:asv-systems}

This work includes the GMM i-vector and x-vector systems in the experiments. Both kinds of systems have two parts: a front-end for utterance-level speaker embedding extraction and a back-end for speaker similarity scoring. The probabilistic linear discriminant analysis (PLDA) back-end is adopted in all the experiments.
% In this work, both i-vector and x-vector systems leverage the probabilistic linear discriminant analysis (PLDA) back-end for similarity scoring. We will introduce these two systems first and then the PLDA back-end.

\subsection{Gaussian Mixture Model i-vector extraction}
% The illustration of gaussian mixture model (GMM) i-vector systems is shown in Figure \ref{fig:gmm-ivector-sys}. Based on the extracted acoustic features, i-vector extractor is used to extract utterance level presentations, i.e. i-vectors. It is composed of two parts, of which one is GMM, and the other one is T-matrix. GMM is used to provide zero and first statistics for i-vector extracting. And T-matrix is a low rank total variability matrix, which maps acoustic feature space into i-vector space. Both GMM and T-matrix are trained on background data. Given the enroll and test i-vectors, probabilistic linear discriminant analysis executes scoring to measure the similarity between them. The higher output score is, the more probable that the two utterances belonging to a same person is.
The illustration of GMM i-vector extractor \cite{dehak2010front} is shown in Fig.~\ref{fig:i-vector-extractor}. It consists of a Gaussian Mixture Model-universal background model (GMM-UBM) and a total variability matrix ($\boldsymbol{T}$ matrix). Given the acoustic features of utterance $i$, GMM-UBM is used to extract the zeroth ($\boldsymbol{N_i}$) and first ($\boldsymbol{\tilde{f_i}}$) order statistics by Baum-Welch statistics computation. The statistics information is incorporated with $\boldsymbol{T}$ matrix to extract i-vector $\boldsymbol{\omega_i}$ as Eq.~\ref{eq:i-vector-extraction},

\begin{equation}
    \boldsymbol{\omega_i} = \boldsymbol{L_i}^{-1}\boldsymbol{T}^\top(\boldsymbol{\Sigma^{(b)}})^{-1}\boldsymbol{\tilde{f_i}}
    \label{eq:i-vector-extraction}
\end{equation}
where $\boldsymbol{L_i} = \boldsymbol{I}+\boldsymbol{T}^\top(\boldsymbol{\Sigma^{(b)}})^{-1}\boldsymbol{N_i}\boldsymbol{T}$, $\boldsymbol{I}$ is the identity matrix and $\boldsymbol{\Sigma^{(b)}}$ is the covariance matrix of GMM-UBM.
% For i-vector eTx matrix is sutraction, a universal background model (UBM) is used to provide zero and first statistics, and the $T$ matrix is a low rank total variability matrix, which maps features from acoustic space into i-vector space. Both GMM-UBM and $T$ matrix parameters are estimated on the training set.

\subsection{x-vector extraction}
% Unlike GMM i-vector systems, x-vector systems leverage the effectiveness of deep neural networks to develop an SV system. The general model architecture is shown in Figure \ref{fig:x-vector-sys}. This x-vector model is trained by speaker recognition task and consists of two parts: frame level and utterance level extractors. On the frame level, acoustic features are fed forward by fully connected (FC) layers. Before each FC layer, a splice layer concatenates the last FC layer's outputs to provide a larger temporal context. On the utterance level, statistics pooling layer aggregates all the frame-level outputs from the last layer and computes its mean and standard deviation. The mean and standard deviation are concatenated together and propagated through utterance-level layers and finally softmax output layer.
% The architecture of the embedding network is shown in Fig.~\ref{fig:x-vector-extractor}.
The x-vector extractor \cite{snyder2018x} leverages DNNs to produce speaker-discriminative embeddings. It consists of frame- and utterance-level extractors. At the frame level, acoustic features are fed forward by several layers of time delay neural network (TDNN). At the utterance level, statistics pooling layer aggregates all the last frame-level layer's outputs and computes their mean and standard deviation. The mean and standard deviation are concatenated together and propagated through utterance-level layers and finally softmax output layer. In the testing stage, given acoustic features of an utterance, the embedding layer output is extracted as the x-vector.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{GMM-ivector-system.png}
%     \caption{The illustration of GMM i-vector system}
%     \label{fig:gmm-ivector-sys}
% \end{figure}

\subsection{Probabilistic linear discriminant analysis back-end}
% Probabilistic linear discriminant analysis (PLDA) is a supervised version of factor analysis \cite{fruchter1954introduction}. Specifically, in our case, it models i-vectors ($x$) by the addition of a global offset $m$, a speaker-specific term $\phi\beta$ and a residual noise $\epsilon_r$, as Equation \ref{eq:plda}. The columns of $\phi$ provides a basis of speaker-specific subspace (eigenvoices), and $\beta$ is a latent identity vector having a standard normal distribution. The residual term $\epsilon_r$ is a guassian distribution with zero mean and a full corvariance matrix $\Sigma$. The EM algorithm is applied to estimate the ML point of model parameters {$m$, $\phi$, $\Sigma$} on training set.
PLDA is a supervised version of factor analysis \cite{fruchter1954introduction}. It models i-vectors/x-vectors ($\boldsymbol{\omega}$) by Eq.~\ref{eq:plda},
% the addition of a global offset $\boldsymbol{m}$, a speaker-specific term $\boldsymbol{\Phi}\boldsymbol{\beta}$ and a residual noise $\boldsymbol{\epsilon_r}$, as Eq.~\ref{eq:plda}. 

\begin{equation}
    \boldsymbol{\omega} = \boldsymbol{m} + \boldsymbol{\Phi}\boldsymbol{\beta} +\boldsymbol{\epsilon_r}
    \label{eq:plda}
\end{equation}
where $\boldsymbol{m}$ is a global bias term, the columns of $\boldsymbol{\Phi}$ provides a basis of speaker-specific subspace, and $\boldsymbol{\beta} \in N(\boldsymbol{0},\boldsymbol{I})$ is a latent speaker-identity vector. The residual term $\boldsymbol{\epsilon_r} \in N(\boldsymbol{0}, \boldsymbol{\Sigma})$ has a Gaussian distribution with zero mean and a full corvariance matrix $\boldsymbol{\Sigma}$. The model parameters \{$\boldsymbol{m}$, $\boldsymbol{\Phi}$, $\boldsymbol{\Sigma}$\} are estimated with the expectation-maximization (EM) algorithm on the training set.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{i-vector-extractor.png}
    \caption{The illustration of GMM i-vector extractor}
    \label{fig:i-vector-extractor}
\end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{x-vector-sys.png}
%     \caption{The illustration of x-vector embedding network}
%     \label{fig:x-vector-extractor}
% \end{figure}


In the testing stage, score $S$ is estimated as a log likelihood ratio of two conditional probabilities (Eq.~\ref{eq:plda-score}). $\boldsymbol{\omega_1}$ and $\boldsymbol{\omega_2}$ are i-vectors/x-vectors extracted from enrollment and testing utterances, respectively. $\mathcal{H}_s$ is the hypothesis that two utterances belong to the same identity, whereas $\mathcal{H}_d$ is the opposite.
\begin{align}
    \nonumber
    S =& \log \frac{P(\boldsymbol{\omega_1},\boldsymbol{\omega_2}|\mathcal{H}_s)}{P(\boldsymbol{\omega_1},\boldsymbol{\omega_2}|\mathcal{H}_d)} \\
          =& \log \frac{P(\boldsymbol{\omega_1},\boldsymbol{\omega_2}|\mathcal{H}_s)}{P(\boldsymbol{\omega_1}|\mathcal{H}_d)P(\boldsymbol{\omega_2}|\mathcal{H}_d)}
    \label{eq:plda-score}
\end{align}


==> adversarial attacks on GMM i-vector based speaker verification systems/conclusion.tex <==
\section{conclusion}
\label{sec:conclusion}
% In this work, we investigate the vulnerability of i-vector based SV models to adversarial attack and its adversarial transferability to NN based SV models. Specifically, FSGM algorithm is applied to generated adversarial audios from GMM i-vector system, and we use these adversarial audios to perform both white and black box attack on GMM i-vector systems and x-vector systems. Experiment results show that one of the most popular non-neural network based model, i.e. GMM i-vector system, is seriously vulnerable to white box attack. Besides, these adversarial audios can further spoof the x-vector systems in terms of black box attack, which is more dangerous in practice. Further work will make effort in developing methods to prevent SV systems from being such adversarial attacks.
In this work, we investigate the vulnerability of GMM i-vector systems to adversarial attacks and the adversarial transferability from i-vector systems to x-vector systems. Experimental results show that GMM i-vector systems are vulnerable to both white and black box attacks. The generated adversarial samples also prove to be transferable to NN speaker embedding based systems, e.g. x-vector systems. Further work will focus on protecting ASV systems against such adversarial attacks, e.g. involving adversarial training strategy to develop ASV systems.


==> adversarial attacks on GMM i-vector based speaker verification systems/experiment_setup.tex <==
\section{Experimental Setup}
\label{sec:exp-setup}

% \subsection{Data set}
The dataset used in this experiment is Voxceleb1 \cite{nagrani2017voxceleb}, which consists of short clips of human speech. There are in total 148,642 utterances for 1251 speakers. Consistent with \cite{nagrani2017voxceleb}, 4874 utterances for 40 speakers are reserved for testing, to generate trials and perform adversarial attacks. The remaining utterances are used for training our SV models. In addition, we apply data augmentation \cite{snyder2018x} when training x-vector embedding networks.
% The training split is used for training our SV models, and the test split is used for generating trials and performing adversarial attacks.

% \subsection{Acoustic features}
Mel-frequency cepstral coefficients (MFCCs) and log power magnitude spectrums (LPMSs) are adopted as acoustic features in this experiment. To extract MFCCs, a pre-emphasis with coefficient of 0.97 is adopted. ``Hamming" window having size of 25ms and step-size of 10ms is applied to extract a frame, and finally 24 cepstral coefficients are kept. For LPMSs, ``blackman" window having size of 8ms and step-size of 4ms is adopted. No pre-emphasis is applied. 

\subsection{ASV model configuration}
In the GMM i-vector system setup, only voice activity detection (VAD) is applied for preprocessing acoustic features. 2048-mixture UBM with full covariance matrix cooperates $\boldsymbol{T}$ matirx with a 400-dimension i-vector space. The i-vectors are centered and length-normalized before PLDA modeling.

% In the x-vector system, cepstral mean and variance normalization (CMVN) and VAD are adopted to preprocess the acoustic features. The x-vector extractor architecture is consistent with \cite{snyder2018x} (Tab.~\ref{tab:x-vector-sys}), where nonlinearities are all rectified linear unites (ReLUs), and $N$ is 1211. The x-vectors are centered and projected using a 200-dimension LDA, and then length-normalized before PLDA modeling.
In the x-vector system, cepstral mean and variance normalization (CMVN) and VAD are adopted to preprocess the acoustic features. The setup of x-vector embedding network is commonly consistent with \cite{snyder2018x}. Extracted x-vectors are centered and projected using a 200-dimension LDA, then length-normalized before PLDA modeling.
% Our implementation code will be available via \textbf{link}.

% In this work, we measure the vulnerability of the systems to adversarial attacks by the degradation of equal error rate (EER) and false acceptance rate (FAR). EER is the rate where acceptance and rejection errors are equal. The FAR threshold is fixed as the EER threshold in the system without attack.

% EER is the rate at which both acceptance and rejection errors are equal, and FAR reflects the prediction error rate over non-target trials when the operation point is fixed at the EER point of original system.

% \begin{table}[t]
% \centering
% \begin{tabular}{c|c|c}
% \hline
%  Layer & Layer Context & Input $\times$ Output \\
%  \hline
%  frame1 & [$t$-2, $t$+2] & 120 $\times$ 512 \\
%  \hline
%  frame2 & \{$t$-2, $t$, $t$+2\} & 1536 $\times$ 512 \\
%  \hline
%  frame3 & \{$t$-3, $t$, $t$+3\} & 1536 $\times$ 512 \\
%  \hline
%  frame4 & \{$t$\}           & 512 $\times$ 512 \\
%  \hline
%  frame5 & \{$t$\}           & 512 $\times$ 1500 \\
%  \hline
%  stats pooling & [0, $T$) & 1500$T$ $\times$ 3000 \\
%  \hline
%  segment6 & \{0\}        & 3000 $\times$ 512 \\
%  \hline
%  segment7 & \{0\}        & 512 $\times$ 512 \\
%  \hline
%  softmax & \{0\} & 512 $\times$ $N$ \\
%  \hline
% \end{tabular}
% \caption{The x-vector extractor architecture. The $N$ in softmax layer is the number of speakers during training. x-vectors are extracted from segment6, before the nonlinearity.}
% \label{tab:x-vector-sys}
% \end{table}
\begin{table*}
\centering
\caption{EER (\%) of the target systems under black box attack with different perturbation degrees ($\epsilon$).}
\begin{tabular}{c|c|c|c|c|c|c|c|c}
\hline
 & $\epsilon = 0$ & $\epsilon = 0.3$ & $\epsilon = 1$ & $\epsilon = 5$ & $\epsilon = 10$ & $\epsilon = 20$ & $\epsilon = 30$ & $\epsilon = 50$ \\
\hline
LPMS-ivec attacks MFCC-ivec  & 7.20 & 8.83 & 13.82 & 50.02 & 69.04 & \textbf{74.62} & 74.59 & 63.24 \\
\hline
MFCC-ivec attacks MFCC-xvec & 6.62 & 8.52 & 14.06 & 57.43 & \textbf{74.32} & 60.85 & 54.07 & 51.34 \\
\hline
LPMS-ivec attacks MFCC-xvec & 6.62 & 7.42 & 9.49 & 25.47 & 37.51 & 43.89 & \textbf{48.48} & 48.39 \\
\hline
\end{tabular}
\label{tab:black-box-attack-eer}
\end{table*}

\begin{table}[t]
\centering
\caption{FAR (\%) of the GMM i-vector systems under white box attack with different perturbation degrees ($\epsilon$).}
\begin{tabular}{c|c|c|c|c|c}
\hline
 & $\epsilon = 0$ & $\epsilon = 0.3$ & $\epsilon = 1$ & $\epsilon = 5$ & $\epsilon = 10$ \\
\hline
MFCC-ivec  & 7.20 & 82.91 & \textbf{96.87} & 18.14 & 16.65 \\
\hline
LPMS-ivec & 10.24 & 96.78 & \textbf{99.99} & 99.64 & 69.95 \\
\hline
\end{tabular}
\label{tab:white-box-attack-far}
\end{table}

\begin{table}[t]
\centering
\caption{EER (\%) of the GMM i-vector systems under white box attack with different perturbation degrees ($\epsilon$).}
\begin{tabular}{c|c|c|c|c|c}
\hline
 & $\epsilon = 0$ & $\epsilon = 0.3$ & $\epsilon = 1$ & $\epsilon = 5$ & $\epsilon = 10$ \\
\hline
MFCC-ivec  & 7.20 & 81.78 & \textbf{97.64} & 50.25 & 50.72 \\
\hline
LPMS-ivec & 10.24 & 94.04 & \textbf{99.95} & 99.77 & 88.6 \\
\hline
\end{tabular}
\label{tab:white-box-attack-eer}
\end{table}

%  The operation point is fixed at the EER point of original system.

% \subsection{Adversarial attack configuration}
% \label{subsec:attack-configuration}
% In this work, we train three ASV models: MFCC based GMM i-vector system (MFCC-ivec), LPMS based GMM i-vector system (LPMS-ivec) and MFCC based x-vector system (MFCC-xvec), and perform white and black box attacks. Two white box attacks are performed on MFCC-ivec and LPMS-ivec systems respectively, and three black box attacks in the mutual attack settings: LPMS-ivec attacks MFCC-ivec (cross feature), MFCC-ivec attacks MFCC-xvec (cross model architecture) and LPMS-ivec attacks MFCC-xvec (cross both). The last two settings is to investigate the adversarial samples' transferability to x-vector systems.
\subsection{Evaluation metrics}
The evaluation metrics of ASV systems could be false rejection rate (FRR), false acceptance rate (FAR) and equal error rate (EER). The FRR and FAR measure the classification error for target and non-target trials, respectively, and EER is the balanced metric where two error rates are equal. As realistic attack situations are mostly similar with non-target trials, we are more concerned with the FAR increase of the system after adversarial attacks. Actually for target trials, instead of adversarial perturbations, simple random noise added to the input could also cause the system to fail in recognizing the owner's voice, so the FRR increase could not reflect the vulnerability of ASV systems to adversarial attacks well. With the considerations above, we measure the system vulnerability to adversarial attacks by the increase of FAR and EER.

\subsection{ABX test}
To evaluate the auditory indistinguishability of adversarial audios compared with the original audios, we perform the ABX test \cite{munson1950standardizing}, which is a forced choice test to identify detectable differences between two choices of sensory stimuli. The adversarial samples are generated from the LPMS-ivec by using FGSM with $\epsilon$ equal to 1. Each adversarial audio is reconstructed from the perturbed LPMSs and the phase of its corresponding original audio. In this work, 50 randomly selected original-adversarial audio (A and B) pairs are presented to the listeners, and from each pair, one audio is chosen as the audio X. Eight listeners join this test, and they are asked to choose one audio from A and B, which is the audio X.

% A subject is presented with two known samples (i.e., A and B) followed by one unknown sample X that is randomly selected from either A or B. The subject is then required to identify X as either A or B. 


==> adversarial attacks on GMM i-vector based speaker verification systems/experiments.tex <==
% \begin{table*}
% \centering
% \begin{tabular}{c|c|c|c|c|c|c|c|c}
% \hline
%  & $\epsilon = 0$ & $\epsilon = 0.3$ & $\epsilon = 1$ & $\epsilon = 5$ & $\epsilon = 10$ & $\epsilon = 20$ & $\epsilon = 30$ & $\epsilon = 50$ \\
% \hline
% cross feature  & 7.20 & 8.83 & 13.82 & 50.02 & 69.04 & \textbf{74.62} & 74.59 & 63.24 \\
% \hline
% cross model architecture & 6.62 & 8.52 & 14.06 & 57.43 & \textbf{74.32} & 60.85 & 54.07 & 51.34 \\
% \hline
% cross both & 6.62 & 7.42 & 9.49 & 25.47 & 37.51 & 43.89 & \textbf{48.48} & 48.39 \\
% \hline
% \end{tabular}
% \caption{Equal error rate (\%) of the target system under different perturbation degree $\epsilon$.}
% \label{tab:black-box-attack-eer}
% \end{table*}

% \begin{table}[t]
% \centering
% \begin{tabular}{c|c|c|c|c|c}
% \hline
%  & $\epsilon = 0$ & $\epsilon = 0.3$ & $\epsilon = 1$ & $\epsilon = 5$ & $\epsilon = 10$ \\
% \hline
% MFCC-ivec  & 7.20 & 81.78 & \textbf{97.64} & 50.25 & 50.72 \\
% \hline
% LPMS-ivec & 10.24 & 94.04 & \textbf{99.95} & 99.77 & 88.6 \\
% \hline
% \end{tabular}
% \caption{Equal error rate (\%) of the GMM i-vector system under different perturbation degree $\epsilon$.}
% \label{tab:white-box-attack-eer}
% \end{table}

% \begin{table}[t]
% \centering
% \begin{tabular}{c|c|c|c|c|c}
% \hline
%  & $\epsilon = 0$ & $\epsilon = 0.3$ & $\epsilon = 1$ & $\epsilon = 5$ & $\epsilon = 10$ \\
% \hline
% MFCC-ivec  & 7.20 & 82.91 & \textbf{96.87} & 18.14 & 16.65 \\
% \hline
% LPMS-ivec & 10.24 & 96.78 & \textbf{99.99} & 99.64 & 69.95 \\
% \hline
% \end{tabular}
% \caption{False rejection rate (\%) of the GMM i-vector system under different perturbation degree $\epsilon$. The operation point is fixed at the EER point of original system.}
% \label{tab:white-box-attack-far}
% \end{table}

\section{experiment results}
\label{sec:experiments}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{black_box_far.png}
    \caption{FAR (\%) of the target systems under black box attack with different perturbation degrees ($\epsilon$).}
    \label{fig:black-box-far}
\end{figure}

% \subsection{Experiment Setup}
% The dataset used in this experiment is Voxceleb1, which consists of short clips of human speech. There are totally over 100,000 utterances for 1251 celebrities. The training split is used for training our SV models, and the test split is used for generating trials and perform adversarial attacks.

% Mel-frequency cepstral coefficients (MFCCs) and log power magnitude spectrum (LPMS) are adopted as acoustic features in this experiment. To extract MFCCs, "hamming" window having size of 25ms and step-size of 10ms is applied to extract a frame. And a pre-emphasis with coefficient of 0.97 is adopted. Finally 24 cepstrals are kept. For LPMS, "blackman" window having size of 8ms and step-size of 4ms is adopted. No pre-emphasis is applied. 

% Two kinds of SV system architectures are adopted in this experiment, as mentioned in Section \ref{sec:asv-systems}. In GMM i-vector system setup, only voice activity detection (VAD) is applied for preprocessing acoustic features. GMM has 2048 components with a full covariance matrix, and the i-vector space has 400 dimensions. In X-vector system, cepstral mean and variance normalization (CMVN) and VAD are adopted to preprocess the acoustic features. The system implement details are shown in Table \ref{tab:x-vector-sys}, which is consistent with \cite{snyder2018x}. The nonlinearities are all rectified linear unites (ReLUs). Both SV systems adopt PLDA as a backend scoring mechanism.

% To evaluate the indistinguishability of adversarial audios compared with the audio they are generated from, we perform an ABX test. ABX test is a method of identifying detectable differences between two choices of sensory stimuli. A subject is presented with two known samples (i.e., A and B) followed by one unknown sample X that is randomly selected from either A or B. The subject is then required to identify X as either A or B. The adversarial signals are generated from GMM i-vector system by using FSGM with $\epsilon$ equal to 1. Each adversarial audio is reconstructed from the perturbed LPMS and the phase spectrum of its corresponding original audio signal. In this experiment, 50 randomly selected original-adversarial audio pairs are presented to listeners, and from each pair one audio is chosen as the audio X. Eight listeners join this test, and they are asked to choose one audio from A and B, which sounds more like the audio X.

% \begin{table}[ht]
% \centering
% \begin{tabular}{c|c|c}
% \hline
%  Layer & Layer Context & Input $\times$ Output \\
%  \hline
%  frame1 & [t-2, t+2] & 120 $\times$ 512 \\
%  \hline
%  frame2 & {t-2, t, t+2} & 1536 $\times$ 512 \\
%  \hline
%  frame3 & {t-3, t, t+3} & 1536 $\times$ 512 \\
%  \hline
%  frame4 & {t}           & 512 $\times$ 512 \\
%  \hline
%  frame5 & {t}           & 512 $\times$ 1500 \\
%  \hline
%  stats pooling & [0, t) & 1500T $\times$ 3000 \\
%  \hline
%  segment6 & {0}        & 3000 $\times$ 512 \\
%  \hline
%  segment7 & {0}        & 512 $\times$ 512 \\
%  \hline
%  softmax & {0} & 512 $\times$ N \\
%  \hline
% \end{tabular}
% \caption{The x-vector DNN architecture. The N in softmax layer is the number of speakers during training. X-vectors are extracted from Layer 6, before the nonlinearity.}
% \label{tab:x-vector-sys}
% \end{table}

\subsection{ABX test results}
Experiment results show that the average accuracy of ABX test is \textbf{51.5\%}, which verifies that human cannot distinguish between the adversarial and corresponding original audios.

\subsection{White box attacks}
We perform the white box attack on both MFCC-ivec and LPMS-ivec systems. The FARs of the two systems under different perturbation degree $\epsilon$ are shown in Table~\ref{tab:white-box-attack-far}. Specifically, the columns where $\epsilon$ equals 0 exhibit the system performance without attack. It is observed that the FARs for both systems are dramatically increased by around 90\% when $\epsilon$ equals 1, where humans still cannot distinguish between the adversarial samples and the original ones. Similar results can be observed in the EER performance of the two systems, as shown in Table~\ref{tab:white-box-attack-eer}. This verifies that GMM i-vector systems are vulnerable to white box attacks. Moreover, from the columns where $\epsilon=5,10$ in Table~\ref{tab:white-box-attack-far} and \ref{tab:white-box-attack-eer}, we also observe that continuously increasing $\epsilon$ beyond some value can decrease attack effectiveness. One possible explanation is that continuously increasing $\epsilon$ makes the perturbations go beyond adversarial effectiveness and simply become noise. Noise cannot degrade ASV systems in terms of non-target trials, so the FARs begin to decrease. But the noise can still degrade ASV systems in terms of target trials, so the balanced metric EER tend to converge to around 50\%. This phenomenon is also observed in the experimental results of black box attacks.

% We perform white box attack on two GMM i-vector systems, i.e. MFCCs and LPMSs based systems. The EERs of the systems under different perturbation degree $\epsilon$ are shown in Table~\ref{tab:white-box-attack-eer}. Especially, the columns where $\epsilon$ equals 0 exhibit the performance of the systems without attack. We observe that both systems are most vulnerable when $\epsilon$ equals 1, where the EERs are both increased by around 90\%. Meanwhile, the FARs of the systems are also shown in Table~\ref{tab:white-box-attack-far}. The FARs of both systems are increased by around 90\% when $\epsilon$ equals 1. These two observations confirm that GMM i-vector systems are vulnerable to white box attack. Another observation is that the attack success rate increases first and then decreases as $\epsilon$ increases, rather than keeps increasing with $\epsilon$. The increase at first (small perturbation) is due to the adversarial perturbation effort, but a large perturbation will bring much difference and mitigate this effort to make the attack success rate down. Technically speaking, the function $S$ (in Eq.~\ref{eq:our-case-0}) w.r.t. the input $\boldsymbol{X}$ is actually non-convex, and a large perturbation breaks the linear approximation of $S$ at point $\boldsymbol{X}$ assumed by FGSM. This will decrease the attack effectiveness.

% increases when $\boldsymbol{X}$ moves a small step in the gradient direction, but theoretically could decrease for a large step due to the non-convexity. The increase/decrease of $S$ directly affects the system's prediction (accept/reject) on the perturbed test utterance, and finally the system performance.

\subsection{Black box attacks}
As configured in Section~\ref{sec:adv-examples-gen}, three black box attack settings are involved, i.e. LPMS-ivec attacks MFCC-ivec (cross-feature), MFCC-ivec  attacks MFCC-xvec (cross-model architecture) and LPMS-ivec attacks MFCC-xvec (cross-feature-model). The FAR fluctuations under these attack settings are illustrated in Fig.~\ref{fig:black-box-far}. It is observed that the FAR is dramatically increased in all three attack settings. Specifically, FAR increases the most by around 60\%, 50\% and 30\% in cross-feature, cross-model architecture and cross-feature-model settings, respectively. The most effective attack appears in the cross-feature setting, while the least effective attack appears in the cross-feature-model setting. This suggests that black box attack effectiveness can be affected by the gap between source and target system settings. The FAR degradation confirms that both GMM i-vector and x-vector systems are vulnerable to black box attacks. Specifically, the adversarial samples crafted from i-vector systems are transferable to x-vector systems. Similar results can be observed in the EER performance, as shown in Table~\ref{tab:black-box-attack-eer}. The phenomenon that x-vector systems are vulnerable to black box attacks also indicates their vulnerability to a more severe attack, i.e. white box attacks.

Moreover, we observe that a large $\epsilon$ value can still make an effective attack, e.g. 20 in the cross-feature setting. 
In this case, humans can perceive a small noise in the spoofing audios, but still confirm that the speaker identity does not change between the original and the corresponding spoofing audios.
% In this case, human could perceive small noise from the spoofing audios, but still confirm the speaker identities behind the spoofing and original audios are the same.
Some adversarial samples and the corresponding system responses are illustrated in this URL\footnote{https://lixucuhk.github.io/adversarial-samples-attacking-ASV-systems}.

% As configured in Section \ref{subsec:attack-configuration}, three black box attack settings are involved, i.e. LPMS-ivec attacks MFCC-ivec (cross feature), MFCC-ivec  attacks MFCC-xvec (cross model architecture) and LPMS-ivec attacks MFCC-xvec (cross both). EERs and FARs are shown in Table~\ref{tab:black-box-attack-eer} and Fig.~\ref{fig:black-box-far} respectively. We observe that EER is increased by 67.42\%, 67.70\% and 41.86\% in the settings of cross feature, cross model architecture and cross both, respectively. Also, FAR is increased by around 60\%, 50\% and 30\% in cross feature, model architecture and both respectively. These observations confirm that both GMM i-vector and x-vector systems are vulnerable to black box attack. And the systems are most fragile to cross-feature attack, while relatively more robust to cross-both attack. We also observe that the $\epsilon$ where the target system is most vulnerable is different due to different source-target attack settings. In some cases, $\epsilon$ increases to a large value to make the most serious attack, e.g. 20 in the cross-feature setting. In this case, the spoofing audio has a noise that human can easily perceive, but human can still confirm the spoofing and original one belong to the same person. Here\footnote{https://lixucuhk.github.io/adversarial-samples-attacking-ASV-systems} are some adversarial samples and the corresponding system responses. Since x-vector systems prove to be vulnerable to black box attack, it suggests that these systems are also vulnerable to a more aggressive attack, i.e. white box attack.

% \begin{table*}
% \centering
% \begin{tabular}{c|c|c|c|c|c|c|c|c}
% \hline
%  & $\epsilon = 0$ & $\epsilon = 0.3$ & $\epsilon = 1$ & $\epsilon = 5$ & $\epsilon = 10$ & $\epsilon = 20$ & $\epsilon = 30$ & $\epsilon = 50$ \\
% \hline
% cross feature  & 7.20 & 8.06 & 10.16 & 23.67 & 30.07 & \textbf{30.82} & 26.78 & 15.1 \\
% \hline
% cross model architecture & 6.62 & 7.56 & 9.96 & \textbf{25.75} & 22.56 & 12.32 & 10.52 & 10.1 \\
% \hline
% cross both & 6.62 & 7.02 & 8.05 & 13.99 & 17.69 & \textbf{18.74} & 17.14 & 13.81 \\
% \hline
% \end{tabular}
% \caption{Equal error rate (\%) of the target system under different perturbation degree $\epsilon$.}
% \label{tab:black-box-attack-eer}
% \end{table*}

% \begin{table}[ht]
% \centering
% \begin{tabular}{c|c|c|c|c|c}
% \hline
%  & $\epsilon = 0$ & $\epsilon = 0.3$ & $\epsilon = 1$ & $\epsilon = 5$ & $\epsilon = 10$ \\
% \hline
% MFCC-ivec  & 7.20 & 43.01 & \textbf{56.61} & 10.9 & 10.41 \\
% \hline
% LPMS-ivec & 10.24 & 62.78 & \textbf{85.67} & 75.24 & 32.83 \\
% \hline
% \end{tabular}
% \caption{Equal error rate (\%) of the GMM i-vector system under different perturbation degree $\epsilon$.}
% \label{tab:white-box-attack-eer}
% \end{table}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.5\textwidth]{white_box_FAR.png}
%     \caption{Caption}
%     \label{fig:white-box-FAR}
% \end{figure}


==> adversarial attacks on GMM i-vector based speaker verification systems/introduction.tex <==
\section{Introduction}
\label{sec:intro}
% Automatic speaker verification (ASV) systems aim at confirming a spoken utterance against an speaker identity claim. It is now a mature technology to be applied in biometric authentication cases, such as voice activation in phones, bank authentication online. Through decades of years developing, speaker verification community has leveraged different modeling technology into this research area. Begin with traditional machine learning models, such as gaussian mixture model-universal background model (GMM-UBM)\cite{reynolds2000speaker}, GMM supervectors based support vector machine (SVM) classifier \cite{campbell2006support} and GMM i-vector systems with probabilistic linear discriminant analysis (PLDA) scoring \cite{dehak2010front,kenny2012small,prince2007probabilistic,garcia2011analysis}, the developed models are more and more robust to channel and speech content information, which are entangled with speaker information in the utterances. With the recent development of deep learning technology, some deep neural network (DNN) based speaker embedding methods proved to be effective in modeling speaker identities, such as d-vectors \cite{variani2014deep} and x-vectors \cite{snyder2018x}. Recently, some end-to-end style DNN based models \cite{zhang2016end,heigold2016end,snyder2016deep} were proposed to directly learn a mapping from enroll-test utterance pairs to verification scores, resulting in a compact structure and comparably good performance.

Automatic speaker verification (ASV) systems aim at confirming a spoken utterance against a speaker identity claim. Through decades of development, the speaker verification community has made great progress and applied this technology in many biometric authentication cases, such as voice activation in electronic devices, ebanking authentication, etc. 
% Automatic speaker verification (ASV) systems aim at confirming a spoken utterance against a speaker identity claim. It has been applied in many biometric authentication cases, such as voice activation in phones, bank authentication online, etc. Through decades of years' development, speaker verification community has made great progress in designing different modeling technologies. 

% However, past research has shown that ASV systems are vulnerable to malicious attacks via spoofing and fake audios, such as imitated \cite{zetterholm2004comparison,wu2015spoofing}, replayed \cite{wu2015spoofing,wu2014study}, synthetic \cite{shchemelinin2013examining,shchemelinin2014vulnerability} and converted  \cite{kinnunen2012vulnerability} speech. These spoofing and fake speech are created with the objective that the speech sounds like the voice of the target person as much as possible. Meanwhile, a lot of research \cite{alegre2013spoofing,todisco2017constant,alegre:hal-00849138} contributed in developing the countermeasures in each case of these attacks. But due to the deviation of human perception and ASV systems, another kind of attacks shows a potential threat to ASV systems: adversarial attacks. Via this attack, the system is spoofed while the spoofing speech still sounds like the voice of the imposter for human perception. This will expose the systems to be dangerously attacked in some situations, such as controlling one's voice-operated devices without his/her awareness.
However, past research has shown that ASV systems are vulnerable to malicious attacks via spoofing speech, such as impersonation \cite{zetterholm2004comparison,wu2015spoofing}, replay \cite{wu2015spoofing,wu2014study}, speech synthesis \cite{shchemelinin2013examining,shchemelinin2014vulnerability} and voice conversion  \cite{kinnunen2012vulnerability}. Among these four types of spoofing attack, replay, speech synthesis and voice conversion pose the most serious threats to ASV systems. The created spoofing speech could sound extremely close to the voice of the target person.
% These spoofing and fake speech are created to sound like the voice of the target person as much as possible. 
Moreover, ASV systems could also be spoofed even though the spoofing speech sounds like the voice of the imposter from human perception. It will expose the systems to some other dangerous situations, such as controlling one's voice-operated devices in place of the real owner unbeknownst to him/her. These threats could be posed by adversarial attacks.

According to \cite{szegedy2013intriguing,ebrahimi2018adversarial,goodfellow2014explaining}, deep neural networks (DNNs) with impressive performance can be vulnerable to simple adversarial attacks in many tasks, such as face recognition \cite{agarwal2018image,sharif2016accessorize}, image classification \cite{liu2016delving,athalye2017synthesizing}, and speech recognition \cite{carlini2018audio}. However, to the best of our knowledge, the only work that applied adversarial attack into ASV systems is \cite{kreuk2018fooling} where they verified the vulnerability of an end-to-end ASV system to adversarial attacks. Briefly, there are three representative ASV frameworks: i-vector speaker embedding based systems \cite{dehak2010front,kenny2012small,prince2007probabilistic,garcia2011analysis}, neural network (NN) speaker embedding based systems \cite{variani2014deep,snyder2018x} and end-to-end approaches \cite{zhang2016end,heigold2016end,snyder2016deep}. While end-to-end based systems have proved to be vulnerable to adversarial attacks, the robustness of other approaches, including GMM i-vector based systems and NN speaker embedding based systems (e.g. x-vector systems we implement), still remains to be explored. GMM i-vector based systems are widely applied to biometric authentication, and it is imperative to investigate their robustness to such adversarial attacks.

% To perform an adversarial attack, a designed small perturbation is added on the input so that the model outputs a wrong prediction while there is no difference between spoofing and original input for human perception. According to \cite{szegedy2013intriguing,carlini2018audio,goodfellow2014explaining}, although DNNs have shown impressive performance in many difficult tasks, such as image classification, speech recognition and machine translation, they also can be vulnerable to adversarial attacks. Many works \cite{carlini2017towards,moosavi2016deepfool,kreuk2018fooling,cisse2017houdini,akhtar2018threat,elsayed2018adversarial} explored this phenomenon and try to improve the robustness of DNNs. However, to the best of our knowledge, the only work that applied adversarial attack into ASV systems is \cite{kreuk2018fooling} where they investigated the robustness of an end-to-end DNN based ASV system under adversarial attacks. While DNN based ASV models have proved to be vulnerable to adversarial attacks, the robustness of traditional ASV models, i.e. non-neural network based models, is still a question to be answered.
Adversarial attacks aim at perturbing the system input in a purposefully designed way to make the system behave incorrectly. The perturbations are usually subtle so that human cannot perceive differences between the adversarial and original inputs. There are two main attack scenarios: white box attack and black box attack. The white box attack allows the attacker to access the complete parameters of the system, so that the system function could be directly involved to optimize the input perturbations. The black box attacker only has the access to the system's input and output, and the adversarial samples are usually crafted by other substitute systems.
% Adversarial attacks have two main scenarios: white box attack and black box attack. White box attack allows the attacker to access the complete parameters of the system, and adversarial samples can be constructed by an optimization on the input while fixing the system parameters. Black box attacker only has the access to the system's input and output, and adversarial samples are crafted by other substitute systems. To generate an adversarial sample, a designed subtle perturbation is added to the input so that the system outputs a wrong prediction while there is nearly no difference from human perception between the spoofing and original input.

% Especially, Gaussian mixture model (GMM) i-vector based systems are non-neural network based models, we can not easily infer their vulnerability to adversarial attacks from previous works.

% Many works explored this phenomenon and tried to improve the robustness of DNNs to adversarial attacks \cite{carlini2017towards,moosavi2016deepfool,kreuk2018fooling,akhtar2018threat,elsayed2018adversarial}.

% In ASV area, some works involve adversarial training to mitigate domain mismatch \cite{bhattacharya2019adapting,bhattacharya2019generative,meng2019adversarial}, improve the system robustness to noise \cite{michelsanti2017conditional,yu2017adversarial}, etc. 

% Carlini et al. \cite{carlini2018audio} exhibit the vulnerability of an automatic speech recognition (ASR) system to adversarial attacks, where the adversarial audios can be transcribed as any phrase. Similar vulnerability of the systems is also proved in image recognition \cite{liu2016delving,athalye2017synthesizing}, machine translation \cite{belinkov2017synthetic,ebrahimi2018adversarial}, etc.

% In ASV area, GMM i-vector system is one of the most powerful traditional models, and its performance is comparable with the state of the art performance of x-vector systems.

For adversarial samples generation, many algorithms were previously proposed to solve the perturbation optimization problem, such as fast gradient sign method (FGSM) \cite{goodfellow2014explaining}, basic iterative method (BIM) \cite{kurakin2016adversarial} and DeepFool \cite{moosavi2016deepfool}. In this work, we simply adopt FGSM to verify the ASV system's vulnerability to adversarial attacks.

This work focuses on the vulnerability of GMM i-vector systems to adversarial attacks, and the transferability of adversarial samples crafted from i-vector systems to x-vector systems. Specifically, we perform both white and black box attacks on GMM i-vector systems and black box attacks on x-vector systems. The detailed attack configurations are illustrated in Section~\ref{sec:adv-examples-gen}. In this work, FGSM \cite{goodfellow2014explaining} is adopted for adversarial perturbations optimization. Our codes have been made open-source\footnote{https://github.com/lixucuhk/adversarial-attack-on-GMM-i-vector-based-speaker-verification-systems}.
% This work focuses on the robustness of GMM i-vector systems under adversarial attacks, and the adversarial samples' transferability to x-vector systems. One of the simplest attack methods, i.e. fast gradient sign method (FGSM) \cite{goodfellow2014explaining}, is adopted to generate adversarial samples from GMM i-vector systems. These samples are used to perform white and black box attacks on GMM i-vector systems, and black box attack on x-vector systems. Our codes were made open-source\footnote{https://github.com/lixucuhk/adversarial-attack-on-GMM-i-vector-based-speaker-verification-systems}.
% The detailed attack configuration is shown in Section \ref{subsec:attack-configuration}.

This paper is organized as follows. Section~\ref{sec:asv-systems} introduces the ASV systems adopted in our experiments. The adversarial attack configurations and the FGSM optimization algorithm are illustrated in Section~\ref{sec:adv-examples-gen}. Section~\ref{sec:exp-setup} and \ref{sec:experiments} describe the experimental setup and results, respectively. Finally, Section~\ref{sec:conclusion} concludes this work.

